Search for B0 -> K*+ K*-

We report the results of a search for the decay B0 -> K*+ K*- with a sample of 454 +/- 5 million BBbar pairs collected with the BaBar detector at the PEP-II asymmetric-energy e+e- collider at the Stanford Linear Accelerator Center. We obtain an upper limit at the 90% confidence level on the branching fraction for Br(B0 -> K*+ K*-) < 2.0 x 10^{-6}, assuming the decay is fully longitudinally polarized.

==> abstract.tex <==
%\documentclass[aps,prl]{revtex4}
%\begin{document}
We report the results of a search for the decay $B^0 \rightarrow K^{*+} K^{*-}$
with a sample of $454\pm5$ million $B\overline{B}$ pairs
collected with the BaBar detector at the PEP-II asymmetric-energy 
$e^+e^-$ collider at the Stanford Linear Accelerator Center. We
 obtain an upper limit at the 90\% confidence level on the branching
fraction for ${\cal B} (B^0 \rightarrow K^{*+} K^{*-}) < 2.0 \times 10^{-6}$,
assuming the decay is fully longitudinally polarized.
%\end{document}


==> runlatex <==
#!/usr/bin/perl
#
# $Id: runlatex,v 1.1 2008/03/17 16:24:06 fwilson Exp $
#
  print  "add_linenum paper.tex\n";
  system "add_linenum paper.tex";

#@inputFiles = `grep -l "begin{document}" *.tex`;
#@inputFiles = `grep -l "begin{document}" paper_linenum.tex abstract.tex`;
@inputFiles = `grep -l "begin{document}" paper.tex  paper_linenum.tex`;


foreach $inputFile (@inputFiles) {

  chomp $inputFile;
  $dviFile = $psFile = $pdfFile = $bibFile = $inputFile;
  $dviFile =~ s/tex/dvi/;
  $bibFile =~ s/\.tex//;
  $psFile =~ s/tex/ps/;
  $pdfFile =~ s/tex/pdf/;

  $landscape = "";
  $docClass = `grep "documentclass" $inputFile`;
  if ($docClass =~ /landscape/) { $landscape = "-t landscape";  }


  print  "latex $inputFile\n";
  system "latex $inputFile";
  print  "bibtex $bibFile\n";
  system "bibtex $bibFile";
  print  "latex $inputFile\n";
  system "latex $inputFile";
  print  "latex $inputFile\n";
  system "latex $inputFile";

  print  "dvips $landscape -Ppdf -o $psFile $dviFile\n";
  system "dvips $landscape -Ppdf -o $psFile $dviFile";
  print  "ps2pdf $psFile $pdfFile\n";
  system "ps2pdf $psFile $pdfFile";
  print  "gzip -f -v --best $psFile\n";
  system "gzip -f -v --best $psFile";

}
print  "rm -f *.log *.dvi *.aux *.toc *.out *.end *.bbl *.blg\n";
system "rm -f *.log *.dvi *.aux *.toc *.out *.end *.bbl *.blg";

